Self-Clustering Hierarchical Multi-Agent Reinforcement Learning with Extensible Cooperation Graph

Multi-Agent Reinforcement Learning (MARL) has been successful in solving many cooperative challenges. However, classic non-hierarchical MARL algorithms still cannot address various complex multi-agent problems that require hierarchical cooperative behaviors. The cooperative knowledge and policies learned in non-hierarchical algorithms are implicit and not interpretable, thereby restricting the integration of existing knowledge. This paper proposes a novel hierarchical MARL model called Hierarchical Cooperation Graph Learning (HCGL) for solving general multi-agent problems. HCGL has three components: a dynamic Extensible Cooperation Graph (ECG) for achieving self-clustering cooperation; a group of graph operators for adjusting the topology of ECG; and an MARL optimizer for training these graph operators. HCGL's key distinction from other MARL models is that the behaviors of agents are guided by the topology of ECG instead of policy neural networks. ECG is a three-layer graph consisting of an agent node layer, a cluster node layer, and a target node layer. To manipulate the ECG topology in response to changing environmental conditions, four graph operators are trained to adjust the edge connections of ECG dynamically. The hierarchical feature of ECG provides a unique approach to merge primitive actions (actions executed by the agents) and cooperative actions (actions executed by the clusters) into a unified action space, allowing us to integrate fundamental cooperative knowledge into an extensible interface. In our experiments, the HCGL model has shown outstanding performance in multi-agent benchmarks with sparse rewards. We also verify that HCGL can easily be transferred to large-scale scenarios with high zero-shot transfer success rates.

==> img/tmp-pdfcrop-24560.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{4353495F696D67312E706466}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> lib/intro-aaai.tex <==
Reinforcement learning has made remarkable achievements in single-agent 
problems such as Atari games.
It also holds promise for solving tasks in multi-agent systems.
Topics within multi-agent systems are diverse as there are many problems 
worth studying.
Most studies follow a paradigm referred to as centralized training with 
decentralized execution(CTDE).
In this paradigm, the agents can access anything during training but
are restricted from making independent decisions during execution.
MADDPG \cite{lowe2017multi} is one of the most classic methods 
that follow this paradigm.
In comparison, the Independently Q-Learning (IQL) \cite{watkins1989learning} 
isolates agent in both training and execution stages.
According to \cite{tampuu2017multiagent}, 
IQL is able to get good scores in some specific tasks 
but the non-stationary issue limits its performance in complex MAS environments.


A considerable amount of literature investigates sparse-reward tasks
and the credit assignment problem behind them.
One of the simplest methods is VDN \cite{sunehag2017value}, 
which assumes that the total Q-value is the sum of individual Q-values.
Qmix \cite{rashid2018qmix} points out that VDN is only able to 
represent a small part of all the possible Q-value decomposition
satisfying Individual-Global-Max (IGM), 
and uses hyper networks to construct an improved decomposition network.
Weighted Qmix \cite{rashid2020weighted}, and QTRAN \cite{son2019qtran} is then
proposed to provide even more general ways of decomposition.
Other studies use difficult approaches to achieve credit assignment.
COMA \cite{foerster2018counterfactual} takes advantage of CTDE and
estimates the counterfactual advantage function to determine the contribution of each agent.
QPD \cite{yang2020q} leverages the integrated gradient to directly decomposite Q-values.

% 注意力系列
Other research branches concentrate on learning more complex cooperative behavior 
to accomplish hard cooperative multi-agent tasks.
These studies usually weaken the constraints of CTDE and 
allow communication even in the execution stage.
In order to aggregate important features from an arbitrary number of agents,
soft attention module \cite{vaswani2017attention} is widely adopted.
In \cite{hoshen2017vain, iqbal2019actor}, 
a centralized critic based on attention module is put forward 
for more precise state value estimation.
Furthermore, 
it is found that the deep graph network \cite{scarselli2008graph} 
is an appropriate media to describe an environment involving multiple agents.
By defining the graph nodes as agents, and edges as agent interaction or communication,
studies \cite{agarwal2019learning, jiang2018graph, deka2021natural} reveal that
the DGN holds considerable promise for solving small-scale hard cooperative problems.
However, most existing studies are designed under small-team settings.
The issues of large-scale multi-agent systems are rarely studied.
In studies of NLP, 
it is found that soft attention has limitations dealing with long sentence sequence \cite{shen2018reinforced}.
When current attention-based RL algorithms are deployed in a rich-agent environment,
a similar performance degradation emerges due to the overwhelmed attention modules.


% 多智能体强化学习环境枚举
In the studies of Q-value decomposition, 
Starcraft micro-management environment 
\cite{vinyals2017starcraft, usunier2016episodic} is widely used,
currently, available maps support up to 27 agents in a team.
Multi-Agent Particle Environment (MAPE) \cite{lowe2017multi}, 
is a simple 2D multi-agent environment with great extensibility.
In most MAPE agent number is usually less than 10 \cite{iqbal2019actor}. 
Another interesting environment is hide-and-seek from \cite{baker2019emergent}, 
in which 2 hiders are trained to protect themselves from 2 seekers 
by using tools obtained from the environment.
The Fortattack environment used in \cite{deka2021natural}
simulates a battle between 2 teams, each with 5 agents.
While there are various multi-agent test environments,
environments supporting at least a hundred agents are very rare.
The environment proposed in \cite{zheng2018magent}
studies the competition of hundreds of agents. Nevertheless, 
it is studied in a discrete 2D grid environment and is oversimplified.
By consulting \cite{lowe2017multi,deka2021natural},
we develop a sophisticated battlefield simulation 
supporting up to 300 agents as the test environment 
called Decentralised Collective Assault (DCA).

In our work, we focus on the decentralized reinforcement learning problem for LMAS.
We put forward the concentration network specialized in LMAS tasks, referred to as ConcNet.
Furthermore, we propose a ConcNet-based policy gradient architecture capable of learning 
LMAS policy from scratch.



==> lib/intro-cgmarl.tex <==
The success of reinforcement learning greatly inspired research in multi-agent systems.
Different from classic single-agent problem such as Go \cite{silver2016mastering} and
RTS game \cite{vinyals2017starcraft, vinyals2019grandmaster},
multi-agent reinforcement learning (MARL) focuses on creating cooperative policy for multiple agents,
e.g. Dota 2 \cite{berner2019dota}, SMAC \cite{usunier2016episodic}, 
multi-robot encirclement \cite{zhang2020multi}
and attacker-defender \cite{wu2021multi}.
However, by carefully tuning environment rewards,
all these tasks and solutions tactfully avoid the sparse reward problem, 
which leads to great difficulty not only in MARL 
but also in classic single-agent RL problems.

There are many reasons that the sparse reward problem must not be treated as a trivial issue in MARL.
Firstly,
reward-tuning is likely to introduce biases 
that mislead agents to learn unexpected cooperative behaviors.
Secondly,
the reward re-designer must be knowledgeable about the task itself
and have enough resources for the environment reverse-engineering.
Thirdly,
reward hand-crafting tricks for one problem are likely to fail in the other one
and are valuable to reward poisoning \cite{rakhsha2021reward}.

Compared with single-agent sparse reward challenges \cite{vinyals2019grandmaster},
MARL sparse reward challenges are fundamentally different in sparsity.
In single-agent problems, 
RL algorithm will eventually achieve decomposition of rewards in the dimension of time (delayed rewards \cite{watkins1989learning}),
in which way the key actions leading to success are reinforced. 
However, rewards are decomposed in the dimension of individuals (for credit assignment) in MARL
\textbf{before} they can be decomposed in the dimension of time.
To highlight this distinction between them,	
we define \textbf{first-order sparsity} (1st-sparsity) to describe the difficulty of single-agent sparse reward problems,
and \textbf{second-order sparsity} (2nd-sparsity) to describe that of MARL sparse reward problems.

Until now,
tools capable of learning sparse-reward multi-agent problems are limited.
A practical solution is exploring general intrinsic rewards \cite{achiam2017surprise}, 
such as curiosity mechanism \cite{still2012information, groth2021curiosity}.
For some specific multi-agent tasks,
it is possible to use curriculum learning \cite{gupta2017cooperative, bengio2009curriculum} to train multiagents starting from a very small scale,
then gradually expand the size of the team.
As another alternative,
imitation learning \cite{reddy2019sqil, vecerik2017leveraging, le2017coordinated} from a huge expert database is an efficient option for resourceful organizations.
But such an approach is restricted by regulations protecting data privacy \cite{pan2019you} and depends heavily on human accuracy.

An additional problem is the limited computational resource.
High-performance servers are expensive, and
agents are usually trained in a simplified environment to improve efficiency.
Some obvious cooperative behaviors are impossible to emerge in RL due to these simplifications.
For example, geese use V-shaped formation in migration to reduce energy costs. 
To learn such formation, 
we need to use energy cost as one of the reward terms and run aerodynamics calculations, 
which might take days to simulate seconds of just a single episode.
This fact reminds us that a framework that
combines emergence agent behaviors with human's prior knowledge about cooperation is absent.
Constructing such a framework can significantly 
reduce the cost of learning the most obvious pattern of cooperation 
when dealing with tasks of real-world relevance.

This paper proposes a distinct approach to solve sparse-reward multi-agent problems.
The inspiration is to reduce the 2nd-sparsity to 1st-sparsity
by introducing prior knowledge about the most fundamental cooperation behaviors.
The answer we put forward is Cooperation Graph Multi-agent Reinforcement Learning (CG-MARL).

The proposed algorithm is established revolving around a three-layer Cooperation Graph,
The first layer is the agent layer, each node representing an individual agent.
The middle layer is composed of clusters, the basic unit to execute cooperative actions.
The last layer is the target layer, and each node is a delegate of a cluster-action.
The Cooperation Graph itself does not consist of neural networks,
instead,
in order to achieve dynamic environment responses, 
it accepts manipulation from a policy neural network, 
which is designed based on attention mechanism \cite{vaswani2017attention} 
and trained by RL optimizers.
The adjustment actions $\vec{\mu}(t)$ provided by this policy neural network 
is used to re-map edges of Cooperation Graph.
Clusters parse instruction from targets' cluster-actions $f$ and 
translate them to original-actions $u$ of individual agents.

==> tex_polish/01-abstract.tex.polish.tex <==
Multi-agent Reinforcement Learning (MARL) has been successful in solving numerous cooperative challenges. However, classic non-hierarchical MARL algorithms still cannot address various complex multi-agent problems that require hierarchical cooperative behaviors. The cooperative knowledge and policies learned in non-hierarchical algorithms are implicit and not interpretable, thereby restricting incorporation of existing knowledge. This paper proposes a novel hierarchical MARL model called Hierarchical Cooperation Graph Learning (HCGL) that aims to solve general multi-agent problems. HCGL features a dynamic graph structure named Extensible Cooperation Graph (ECG), which is essential for achieving agents' self-clustering behaviors and hierarchical cooperation. ECG comprises three hierarchical layers consisting of agent nodes, cluster nodes and target nodes, respectively. The primary distinction of our ECG model is that the behavior of agents is directed by the topology of ECG rather than neural policy networks. In this paper, we propose a distinctive approach to manipulate the ECG topology in response to changing environmental conditions. Specifically, we introduce four virtual operators trained to modify the edge connections of the ECG, thereby grouping agents into clusters and achieving higher-level cooperative behaviors. The hierarchical feature of ECG provides a unique approach to merge raw agent actions (executed by individual agents) and cooperative actions (executed by agent clusters) into one unified action space, allowing us to incorporate fundamental cooperative knowledge into an extensible interface. In our experiments, the HCGL model has shown outstanding performance in multi-agent benchmarks with sparse rewards. We also verify that HCGL can easily be transferred to large-scale scenarios with a high zero-shot transfer success rate.

==> tex_polish/02-intro.tex.polish.tex <==
\section{Introduction}

Multi-Agent Reinforcement Learning (MARL) has become increasingly important in establishing cooperative agent strategies within large-scale multi-agent systems. By leveraging deep neural networks, MARL algorithms can extract vital features from large observation spaces and perform sophisticated cooperative behaviors. However, the performance of MARL algorithms is limited by various factors existing in the MARL learning frameworks, particularly when there are a large number of agents \cite{fu2022concentration}. Exploring feasible cooperation strategies under these circumstances is difficult and computationally expensive, even if some of these strategies seem basic or obvious to humans.

Prior studies have explored the application of intrinsic reward \cite{jaques2019social}, reward decomposition \cite{rashid2018qmix}, and other methods. However, reward decomposition shows state-of-the-art performance in small-scale multi-agent tasks, but it performs poorly in scenarios with a large number of agents. On the other hand, the intrinsic reward methods can effectively promote the coverage speed of cooperative behaviors. Nevertheless, the intrinsic reward may introduce biased cognition on tasks from reward designers, leading the agents to learn unexpected behaviors that may not align with the initial objectives. Moreover, reward-shaping techniques that work well for one problem may turn out to be ineffective for another and may even result in reward poisoning \cite{rakhsha2021reward}.

Learning high-level cooperative behaviors in large-scale multi-agent environments is still an open question with the following problems:

\begin{enumerate}
    \item Large-scale multi-agent policy exploration problem: As the joint action space expands dramatically with the number of agents, it grows extremely difficult to explore enough feasible policies for agents to escape from local suboptimal solutions. This problem can be even more severe in environments where rewards are sparse.
    \item Knowledge incorporation problem: Only a limited number of studies investigate blending knowledge into MARL algorithms. A framework that enables knowledge integration is critical for two significant reasons. Firstly, integrating data and models we already possess can significantly enhance RL performance. Secondly, knowledge integration is necessary to learn cooperative behaviors beyond the limitations of RL. Some cooperative behaviors are established based on environmental factors that cannot be easily simulated. For example, birds' formation behavior is based on aerodynamic factors that help them save energy during long flights. Without expensive aerodynamics calculations, RL agents cannot learn even the simplest flight formation as nothing drives them to do so. 
    \item Interpretability problem: Agents in non-hierarchical frameworks learn advanced high-level policies with neural networks, which cannot be easily interpreted. If agents fail to exhibit expected cooperative behaviors after training, diagnosing problems within the agents' policy neural networks is almost impossible.
\end{enumerate}

This paper proposes Hierarchical Cooperation Graph Learning (HCGL) to address these problems:

\begin{enumerate}
    \item Firstly, the joint policy exploration problem can be addressed by introducing a general hierarchical control model. In this paper, HCGL introduces the Extensible Cooperation Graph (ECG), a unique control structure that aims to enable hierarchical multi-agent cooperation while minimizing ineffective exploration behaviors. Different from classic MARL algorithms, agents in HCGL are directly controlled by ECG instead of neural network policies; their action depends solely on the topology of ECG. ECG represents agents as nodes and groups agent nodes into several clusters. Then, each cluster is connected to a series of target nodes defined by either \textit{cooperative actions} (cluster-level actions) or \textit{primitive actions} (agent-level actions). The cooperative actions are high-level actions that are executed by all member agents in a cluster.
    
    \item Secondly, HCGL employs cooperative actions to blend cooperative knowledge into the learning framework. We program basic cooperative behaviors, such as agent gathering and joint attacking, as cooperative actions in ECG. Moreover, we unify both the primitive actions and the cooperative actions into the ECG graph with ECG target node, which fosters the seamless integration of both multi-agent reinforcement learning (MARL) and expert knowledge.

    \item Thirdly, ECG is a graph structure that naturally has stronger interpretability. It is easy to visualize and monitor the cooperative behavior of agents simply by observing the topology of ECG.
\end{enumerate}Finally, HCGL employs four graph operators, which are a group of virtual agents, to dynamically manipulate the ECG edge connections and change the topology of the ECG in real-time. Since the environment is dynamically changing when agents carry out their cooperative operations, it is necessary to adjust the topology of the ECG in response to the environment. To avoid ambiguity with real agents, in the following sections, we will refer to these virtual ECG agents only as graph \textit{operators}. Each graph operator possesses a policy neural network that is trained by a MAPPO \cite{yu2021surprising} RL learner whose sole goal is to maximize the reward of the entire multi-agent team. These graph operators drive the cooperation graph to make adjustments and adaptations according to the changing environments, thus guiding agents to accomplish their objectives.

The main contributions of this study are fourfold: (1) We propose a novel hierarchical graph-based HCGL model with knowledge incorporation capability. (2) We present an approach to visually interpret the behavior of agents with the topology of ECG. (3) We demonstrate the effectiveness of ECG in large-scale cooperative tasks. (4) We show that HCGL efficiently transfers policies learned in small-scale tasks to large-scale ones.

In the following sections, we first introduce related works on prior hierarchical single-agent RL and multi-agent RL. Then we introduce our ECG framework, beginning with the structure of a static cooperation graph. Next, we emphasize how graph operators manipulate the graph to make it dynamic and responsive. Finally, we perform solid experiments to justify the effectiveness of HCGL in different large-scale multi-agent environments.

==> tex_polish/03-related.tex.polish.tex <==
\section{Related Works}

Research on multi-agent systems has been greatly inspired by the success of reinforcement learning. 
Unlike single-agent problems such as Go \cite{silver2016mastering} and RTS game \cite{vinyals2017starcraft, vinyals2019grandmaster}, 
multi-agent reinforcement learning (MARL) focuses on the development of cooperative policies among multiple agents.
The coordination among multiple agents poses a critical challenge in multi-agent learning where agents engage in dynamic interactions to achieve a shared objective (e.g., Dota 2 \cite{berner2019dota}, SMAC \cite{usunier2016episodic}, multi-robot encirclement \cite{zhang2020multi}, and attacker-defender \cite{wu2021multi} scenarios).

Recent studies suggest that achieving multi-agent coordination becomes progressively difficult as the number of agents increases \cite{samvelyan2019starcraft}. While algorithms such as Qmix \cite{rashid2018qmix}, QTRAN \cite{son2019qtran}, COMA \cite{foerster2018counterfactual}, ROMA \cite{wang2020roma}, and ACE \cite{li2022ace} achieve significant success in small and medium-scale multi-agent problems, it is discovered that existing MARL methods have many limitations in large-scale cooperative tasks. For example, as the team size expands, it becomes challenging to accurately distribute rewards among individual agents. Moreover, an increase in the joint policy space exacerbates the difficulty of exploring agent actions. Therefore, it is imperative to investigate alternative approaches to tackle large-scale coordination problems. Examples of such attempts include hierarchical multi-agent reinforcement learning (Hierarchical-MARL), multi-agent curriculum learning \cite{wang2021survey}, and knowledge incorporation.

Hierarchical multi-agent reinforcement learning has gained popularity as a research area due to its capacity to address complex problems by partitioning them into sub-problems. These methods usually improve the learning efficiency by re-engineering the agents' action space. A study by Spatharis et al. \cite{spatharis2021hierarchical} proposes a hierarchical multi-agent reinforcement learning scheme for air traffic management that divides the task into two levels: tactical and strategic. Similarly, Singh et al. \cite{singh2020hierarchical} extend this work to maritime traffic management, which models ships as individual agents and the VTS (vessel traffic service) as a regulatory agent. Other works extend this technique to air combat \cite{kong2022hierarchical}, UAV swarm confrontation \cite{wang2021uav, yue2022unmanned}, and football simulations \cite{yang2019hierarchical}. However, most of these methods are task-specific and lack further generalization capability.

Multi-agent curriculum learning aims to address difficult multi-agent problems by learning easier tasks and increasing the difficulty according to a schedule. For example, start off by learning in a multi-agent setting with a limited number of agents, and then gradually and automatically increase the number of agents \cite{zhang2022automatic, wang2020few}. This technique provides a solid solution to solve sparse-reward cooperative multi-agent problems \cite{chen2021variational}. The potential applications of curriculum learning include autonomous driving \cite{yang2021diverse}, SMAC \cite{wang2021uav, yue2022unmanned}, etc.

Another alternative approach is incorporating prior knowledge into the learning algorithm. Deng et al. \cite{deng2020integrating} discussed a variety of ways to use general human knowledge to facilitate reinforcement learning. Singla et al. \cite{singla2019memory} proposes a memory-based RL model that associates the learning process with environmental knowledge to solve UAV obstacle avoidance problems during navigation. Han et al. \cite{han2020improving} suggest a new strategy for enhancing the efficiency of multi-agent reinforcement learning by employing logic rules, a prevalent form of human knowledge, to address SMAC challenges. A more general form of the knowledge-driven approach is knowledge graph reasoning, which is used in other RL problems such as recommendation \cite{xian2019reinforcement, wang2022multi}.

==> tex_polish/04-method.tex.polish.tex <==
\section{Extensible Cooperation Graph}
\begin{figure}[!t] 
    \centering
    \includegraphics[width=\linewidth]{img/ECG_main.pdf}
    \caption{
        An illustration of the Extensible Cooperation Graph (ECG).
        Starting from the bottom, 
        the ECG is a three-layer hierarchical graph structure that includes agent nodes,
        cluster nodes, and target nodes.
        The graph nodes are connected by edges.
        Within each episode,
        this graph will be dynamically controlled by four virtual agents referred to as operators.
    }
    \label{fig:ECG_main}
\end{figure}


We first introduce the core structure of our model: the Extensible Cooperation Graph (ECG).
The ECG is a multi-layer non-neural graph with a simple topology (directed and acyclic).
It acts as a mastermind to control the collective behavior of agents 
by changing its own edge connections dynamically.
A basic ECG $G$ contains 3 layers: the agent layer ($\mathcal{A}$), 
cluster layer ($\mathcal{C}$), and target layer ($\mathcal{T}$), respectively.




An agent node $a_i \in \mathcal{A}$ represents an agent in the environment.
Unlike any other MARL algorithm,
each agent in the graph acts as a pawn and does not possess a policy neural network of its own.
Instead,
the behavior of agents depends on the dynamic graph structure and edge connections 
(which will be discussed in the next section).



The cluster nodes are responsible for dividing agents into groups,
which organize agents to complete difficult multi-agent task objectives.
A cluster node $c_k \in \mathcal{C}$ can contain all agents when needed.
On the other hand, each agent is required to join only one cluster at a specific time step.
When an agent $a_i$ joins a cluster $c_k$,
we use a directed edge in the ECG to represent this relationship $(a_i, c_k)$.




The target nodes represent special actions that need to be executed by clusters.
The graph relationship of clusters and targets is very similar to that of agents and clusters,
and each cluster chooses one of the targets to follow at each time step.
When a cluster $c_k$ selects a target $t_\tau \in \mathcal{T}$,
an edge is established directing from itself towards the target $(c_k, t_\tau)$.
There are two types of target nodes: raw-action nodes and coop-action nodes.

We introduce raw-action nodes as the first type of target nodes.
Each action from the original agent action space $\mathcal{U}$ is represented as a target node in the ECG.
When a cluster is connected to a raw-action target node,
all of its member agents perform the corresponding raw-action simultaneously.
In other words,
the raw-action is broadcasted from its target node to all connected clusters,
and eventually to all agents connected.

Next, we introduce coop-actions (cooperative cluster actions), the second type of target nodes.
Unlike raw-actions from the original agent action space $\mathcal{U}$,
coop-actions are executed by clusters instead of agents.
Consequently, 
a coop-action can simultaneously affect all agents in a cluster.
When a cluster is connected to a coop-action target node,
the cluster needs to parse the coop-action first according to the status of its member agents,
translating coop-actions into raw-actions for each individual agent 
before finally distributing the resulting raw-actions to each member agent.
As an example, 
``gathering'' and ``scattering'' are two simple coop-actions.
When a cluster is performing the ``gathering'' action,
this coop-action is translated to primitive actions that move each agent towards its allies.
And the ``scattering'' coop-action plays the opposite role and moves agents away from one another.
The same coop-action is usually interpreted into different primitive actions 
for different agents within a cluster.





Coop-actions are essential for integrating cooperative knowledge into the MARL framework.
Without the participation of coop-action target nodes,
learning joint actions like gathering can be time-consuming 
if agents are not guided by dense rewards from the environment.
And even if agents finally learn to perform similar skills, 
the policies still lack transparency and interpretability.
The introduction of coop-actions provides a framework where
knowledge-based joint behaviors 
have the opportunity to take part in the policy optimization process.
Moreover,
since the edge connection of the ECG is dynamic and 
the adjustment policies are gradually optimized during the learning session,
the framework tolerates not only the co-existence of primitive actions and coop-actions,
but also the co-existence of different coop-actions with conflictions.
Detrimental coop-actions can be easily eliminated during learning
by treating them as unwelcomed nodes.Furthermore, the ECG framework provides a compromise between pure RL methods and pure pre-programming methods (rule-based). Many abstract cooperative behaviors, such as "joint attacking" and "rallying at a certain location," from rule-based methods, can be utilized as coop-actions in ECG. At the same time, these coop-actions share an equal position with the primitive-actions in ECG. This means that if a coop-action is not helpful in addressing the problem in the current environment, the corresponding node will be gradually given up during reinforcement learning.

\section{Hierarchical Knowledge Embedding}

In our HCGL model, target nodes are the main media to integrate knowledge with MARL. There are two types of target nodes that represent the cooperative actions and the primitive actions, respectively.

The primitive action corresponds to actions in classic MARL algorithms, where agents need to choose one of the primitive actions to interact with the environment. Cooperative action, on the other hand, is a new concept proposed in HCGL, and it differs from primitive actions in multiple ways. First and most importantly, these actions are executed by clusters rather than agents. A cooperative action guides the collective behavior of all agents in the cluster executing it, for example, making a group of agents maneuver and generate a formation. Secondly, each cooperative action is programmed with expert knowledge, allowing us to integrate low-level cooperative skills into the reinforcement learning framework. Thirdly, the cluster nodes will eventually translate each cooperation action into different primitive actions for each agent individually, considering the purpose of the cooperation action and the state of agents in the cluster.

From the perspective of ECG, when a cluster node is connected to a primitive action, the primitive action will be passed to all agents linked to this cluster unchanged. In comparison, when a cluster node is connected to a cooperative action, the cooperative action is first translated to primitive actions before being delivered to each agent.

The introduction of cooperative actions enables a variety of ways to incorporate expert knowledge:

\begin{itemize}
    \item Employing basic cooperation knowledge such as gathering, scattering, encirclement, following, patrolling, etc. These cooperative behaviors are not only simple but also general in a variety of tasks. Unfortunately, learning these simple behavior may take millions of steps in non-hierarchical RL models. In comparison, it only takes a few lines of code to write a robust controller to achieve these basic behaviors. In HCGL, we program these basic behaviors as cooperative actions to accelerate the learning process.
    \item Applying additional constraints such as flight formation, collision avoidance, keeping communication range, etc. Agents trained in simulations often deviate from our expectations because many factors are not considered in the simulation environments. For example, although we have the knowledge that a V-shaped flight formation can reduce flight energy costs, this behavior cannot be learned unless we consider aerodynamic factors in the simulation. Likewise, many simulation environments do not detect collisions to reduce computational costs, and meanwhile, there are many existing collision avoidance controllers that can be leveraged. In such cases, our HCGL model can take full advantage of these existing algorithms and make them an integrated part of the multi-agent cooperation policy.
\end{itemize}

Note that the HCGL model not only passively incorporates knowledge-based cooperative actions but also actively evaluates, chooses, and switches between them. If some cooperative actions are useless, detrimental, or conflict with one another, the effectiveness of HCGL is not significantly impacted because the topology of ECG is adjusted by graph operators. The graph operators can distinguish detrimental actions and disconnect clusters from these action nodes during the MARL training stage. The following section introduces the method for adjusting ECG.

\section{Learning Graph Manipulation}

As we have mentioned in the previous sections, the agents (agent nodes) do not possess a policy neural network; they only receive directions from the ECG, which must change itself dynamically in each episode. The adjustment of ECG will be carried out by a group of virtual agents referred to as Graph Operators. To distinguish them from other regular agents manipulated inside ECG, we will refer to them only as \textbf{operators} for clarity. There are always four operators to jointly manipulate a ECG. Two of them ($o_{p1}$, $o_{p2}$) are responsible for adjusting the edges between agents and clusters, while the other two ($o_{p3}$, $o_{p4}$) are responsible for adjusting the edges between clusters and targets.The graph operators have a special action space since their job is to manipulate the ECG rather than directly interact with the environment. To transfer an agent from one cluster $c_m$ to another cluster $c_n$, operators $o_{p1}$ and $o_{p2}$ must work together to produce $m \in |\mathcal{C}|$ and $n \in |\mathcal{C}|$, respectively. There are two special cases. First, if operator $o_{p1}$ chooses a cluster that is currently empty (with no agent nodes linking to it), the action of $o_{p1}$ and $o_{p2}$ is invalid, regardless of the action of $o_{p2}$. Second, if operator $o_{p1}$ and $o_{p2}$ happen to choose the same cluster, their action is invalid.

Similarly, the action space of the other two operators, $o_{p3}$ and $o_{p4}$, controls the edges between clusters and targets in the same way. Operators $o_{p3}$ and $o_{p4}$ produce a pair of actions to transfer a cluster linked with target node $t_m$ to a different target node $t_n$, where $m \in |\mathcal{T}|$ and $n \in |\mathcal{T}|$. Again, if no cluster is currently connected to $t_m$ or if $t_m$ and $t_n$ are the same target, this action pair is invalid.

As the number of target nodes is significantly greater than the number of clusters, the operators are likely to spend much time exploring action combinations that are ineffective. To address this issue, we perform action masking to forbid operators from choosing invalid actions by providing operators with their current available actions. This regulation is imposed on $p_{1}$ and $p_{3}$.

\section{Training Graph Operators}
\subsection{Training Operators}

Graph operators are trained with multi-agent RL methods MAPPO, which treat operators (instead of agent nodes) as \textbf{agents}. Like many other multi-agent systems, each graph operator has its own policy network with shared parameters. As illustrated in Fig. \ref{fig:PolicyNetwork}, most policy network parameters are shared among graph operators. Nevertheless, each operator possesses a unique policy head to produce different graph manipulation actions.

We previously introduced that operator actions are only valid when considered in pairs, so it is important that an operator is aware of the action of its fellow operators before making the final action decision. Inspired by ACE \cite{li2022ace}, in our model, the operators sequentially select their actions at each step. Operator 1 (op.1) is the first operator to select an action. When op.2 determines its own action, it refers to the action of op.1. Similarly, op.3 and op.4 take all previous operator actions into consideration when selecting their own actions.

\subsection{Initialization of ECG}

Operators must learn to manipulate ECG differently to generate distinct ECG topologies to perform different cooperative actions. However, the initial ECG topology in each episode still needs to be determined. We adopt the method introduced in \cite{fu2022cooperation}, where the ECG initial topology is generated randomly at the beginning of training. Then, this topology is frozen as the initial state of ECG for all future episodes.

As suggested by \cite{fu2022cooperation}, although the initialization of ECG topology is random, we can still improve the stability of the model by producing multiple random topologies and then choosing one of them according to the entropy of the edge connections. This is because there may exist multiple sub-optimal topologies across all possible ECG structures. We can measure the distance between topologies in terms of the number of operator steps required to complete the transition between two topologies. A high-entropy initial topology can increase its distance from sub-optimal topologies, encouraging graph operators to conduct more exploration before converging. A more comprehensive exploration can aid graph operators in identifying optimal policies more efficiently.

\subsection{Operator Policy Stability Enhancement.}

Operators have significant privileges in our model, as they can alter the behavior of the entire team with minimal effort. This feature of ECG offers considerable hierarchical advantages concerning the training of agents. However, it may potentially weaken the connection between the environment and graph operators.We propose two improvements to enhance the bound between graph operators and the external environment. 

On one hand, we introduce an autoencoder to connect the operator observation input and the representation produced by the last parameter-sharing layer. A typical autoencoder has an encoder that maps input to a low-dimensional space and a decoder that reverses the encoding process to estimate the original input from the low-dimensional representation. In this model, the parameter-sharing feed-forward policy layers perform the role of encoder, and we only need to add an additional decoder to map the final representation to estimate the original operator observations. The loss function (mean squared error) $\mathcal{L}_{ae}$ (together with policy gradient loss) is applied during policy network update.

On the other hand, we generate interference on ECG by altering the ECG edge connections against the action of operators. Similar to the dropout technique utilized in other machine learning problems, interference is applied randomly at the start of every step with a small probability denoted by $p_i$. We select $p_i=0.5$. More specifically, a set of random but fake operator actions is produced and applied to the ECG when interference is triggered. With the participation of interference, operators are forced to learn to reverse the influence caused by fake operator actions. Moreover, this technique motivates operators to learn to analyze the representation of ECG, facilitating the ability to understand the relationship between the environment and ECG itself.

In our ECG model, the graph operator agents (instead of environment agents) are trained by reinforcement learning. As a result, the training process differs slightly from a typical actor-critic RL model. Graph operators gather available information on all nodes in ECG, including agent nodes, cluster nodes, target nodes, and ECG's edge connection. As illustrated in Fig. \ref{fig:PolicyNetwork}, the raw representation of agent nodes is simply the observation of each agent. The raw representation of clusters is one-hot vectors. The raw representation of each target node includes available information about this target. If the target node is a primitive-action, its representation is onehot, and if the target node is a coop-action, we place information about this coop-action instead of onehot coding. For instance, if the coop-action concerns a rally point, we can place the location of this point into the raw representation.

As shown in Fig. \ref{fig:PolicyNetwork}, the representations of targets, clusters, and agents are normalized and then projected into embeddings with fixed dimensions, respectively. Next, we compute attention between cluster nodes and agent nodes (Attention-AC) and cluster nodes and target nodes (Attention-CT). In this step, we take the representation of clusters, the most essential elements of ECG, as attention queries, and the representations of agent nodes as well as target nodes as attention keys. More specifically, both attention layers are cluster-oriented. Attention-AC captures the graph relationship between agents and clusters, combining the representation of each agent with the representation of clusters. On the other hand, Attention-CT captures the graph relationship between targets and clusters, gathering the feature from target nodes to cluster nodes. Then the attention results from Attention-AC and Attention-CT are concatenated and further processed by a Fully Connected (FC) layer, which extracts an embedding $e_h$ that holds a comprehensive ECG representation. The resulting $e_h$ values are eventually utilized for three tasks: (1) estimating the state value, (2) estimating the action logits, and (3) reconstructing the raw node representation using the decoder component of the autoencoder.

For purposes (1) and (2), the embedding of all clusters will be concatenated together, then produce a low-dimension embedding via FC layers. The critic uses this embedding to produce the state value estimation. Each graph operator also uses this embedding sequentially to determine the operator action (also via FC layers).

For purpose (3), we reconstruct raw node representations with additional attention layers: Attention-AE-A, Attention-AE-C, and Attention-AE-T. Using one-hot vectors as query and $e_h$ as keys, we compute the reconstructed agent node representations with Attention-AE-A, then obtain the reconstruction loss with MSE. The reconstruction loss of clusters (reconstructing with Attention-AE-C) and targets (using Attention-AE-T) is produced likewise.

We successfully scaled ECG by the curriculum learning approach. ECG's scaling capability is excellent and has significant advantages when used together with curriculum learning techniques, as shown in Fig. \ref{fig:GraphExtension}.This section proposes a curriculum learning method that leverages the extensibility of ECG to handle large-scale multi-agent problems. The method starts with simple environments featuring fewer agents and gradually transfers to complex environments requiring a large number of agents.

ECG supports the expansion of graph by converting its agent nodes to secondary cluster nodes. Unlike its predecessor agent node that only controls a single agent, a secondary cluster node connects 2 or even more agents, thus expanding the size of the team several times larger. After the expansion, the graph between targets and clusters and the policy of op.3 and op.4 stay unchanged. Op.1 and op.2 are now responsible for controlling the edge between clusters and secondary clusters, using the same policy they learned in the smaller scale environment. Finally, the connection between secondary clusters and the expanded agent team is considered static in ECG; this part of the graph will not be adjusted like the rest of ECG.

The change in ECG also impacts the observation of the policy network of operators. The secondary cluster now connects to the observation of multiple agents rather than a single one. However, the policy network of graph operators still accepts same-shape observation from only one node. In order to successfully transfer the policy parameters learned in the previous task to the larger scale new task, we add an extra attention layer at the beginning of the policy network to merge the observation embeddings of all agents connected to a secondary cluster into one. The initial parameters of the new attention layer are randomly initialized. In contrast, the parameters of the rest of the network inherit from the previous policy network learned in the previous environment.

Like most curriculum learning scenarios, it is likely that the policy of operators learned in the previous environment is not fully capable of commanding agents in a larger team. Moreover, the new attention layer added for compatibility also requires further training. Thus, building on the ones learned in previous scenarios, operators need to learn new adaptive policies and further optimize their policies with RL.

==> tex_polish/05-experiment.tex.polish.tex <==
\section{Simulations}

In this section, we evaluate the performance of HCGL in the Cooperative Swarm Interception benchmark and compare it with existing MARL algorithms. The algorithms evaluated are:

\begin{itemize}
    \item HCGL. The proposed method in this paper. It has two primary hyper-parameters, namely the number of clusters and selection of cooperative actions.
    \item Qmix \cite{rashid2018qmix}. A value-based MARL algorithm that leverages the Individual-Global-Max (IGM) principle and proposes a reward decomposition method. Qmix has state-of-the-art (SOTA) performance in multiple MARL baselines.
    \item Qtran \cite{son2019qtran}. Qtran improves Qmix by providing more general ways of decomposition.
    \item Qplex \cite{wang2020qplex}. Qplex proposes a duplex dueling network architecture to factorize the joint value function.
\end{itemize}

\subsection{Cooperative Swarm Interception}

We evaluate the effectiveness of our ECG model using a sparse reward benchmark called Cooperative Swarm Interception (CSI). The scenario involves a team of defender agents that must prevent multiple hostile invasions from destroying their bases. As illustrated in Figure \ref{CSI}, an invader can be slowed down when it is surrounded by a sufficient number of agents. Moreover, if the number of agents tracking an invader surpasses a specific threshold, the invader is compelled to change its direction away from its target, thus neutralizing the threat of the invader. For example, CSI-54/6/9 denotes that there are 54 defender agents to intercept nine invaders, and each invader can be forced to turn back by at least six agents.

The CSI benchmark uses an extremely sparse benchmark. The agents are rewarded +1 as a team when all bases survive the attackThis section seems to be formatted incorrectly. The first part appears to be the caption and labeling of a figure, while the second part is a table with descriptions of MARL methods. Some modifications are required. 

For the first part, the figures are labeled, but the caption is incomplete. Here is a proofread version:

\begin{figure}[!t]
\centering
\begin{subfigure}{.49\linewidth}
\centering
\includegraphics[width=\linewidth]{img/ecg3.jpg} 
\caption{
ECG topology at step 90.
}
\label{fig:c}
\end{subfigure}
\begin{subfigure}{.49\linewidth}
\centering
\includegraphics[width=\linewidth]{img/ecg4.jpg} 
\caption{
ECG topology at step 130.
}
\label{fig:d}
\end{subfigure}
\caption{ECG topology in an episode in task CSI-27/3/9.
The positioning of the nodes in the figure is as follows: 
Agent nodes are depicted in red and positioned at the bottom, 
Cluster nodes are shown in blue and positioned in the middle, 
while Target nodes are illustrated in green and positioned at the top.
The edge connections are represented by blue and yellow lines in this figure.
}
\label{fig:topology}
\end{figure}

For the second part, it appears to be a table comparing different MARL methods. Here is a proofread version:

This experiment evaluates the performance of HCGL with the CSI benchmark and compares it to other SOTA methods. The success rate metric is used for assessing the performance of algorithms.

The results are displayed in Table \ref{sample-table}. Although we tried multiple hyperparameter settings, Qtran, Qplex, and Qmix methods were unable to solve the CSI benchmark problem at all. Our HCGL, on the other hand, achieved a success rate of 0.97 $\pm$0.03, which significantly outperforms previous methods.

Table \ref{sample-table} compares HCGL's performance to other MARL baselines. The success rates are measured for two scenarios, zero-shot, and final. The latter refers to after the methods are trained and tested on the same scenarios multiple times. HCGL performs significantly better on both occasions. 

Moreover, we tested the transferability of HCGL's policy to other scenarios. Figure \ref{fig:Transferability} shows how the trained policy from CSI-27/3/9 was transferred to CSI-54/6/9, CSI-108/12/9, and so on.Benefits of the Hierarchical ECG Structure

The Hierarchical Clustered Graph Learning (HCGL) model has shown significant transferability benefits for large-scale multi-agent environments involving hundreds of agents due to its hierarchical ECG structure. One of the limitations of non-hierarchical multi-agent reinforcement methods is their poor performance in transferability. Most existing Multi-Agent Reinforcement Learning (MARL) algorithms must be retrained when the number of agents changes due to their policy parameters being related to the number of agents. Previous studies have attempted to improve compatibility by leveraging the transformer structure or attentional graph network. However, a non-hierarchical structure is insufficient for transferability when the number of agents increases twofold or threefold.

In this simulation, we first train the policy in CSI-27/3/9 from scratch and transfer the trained policy to CSI-54/6/9, CSI-81/9/9, CSI-108/12/9, and CSI-216/24/9. The training process is depicted in Fig.\ref{fig:Transferability}, and the result is displayed in Table \ref{sample-table}. The transferred methods are denoted by the suffix "TF" in Table \ref{sample-table}. We evaluate model transferability with two metrics: the zero-shot success rate and final success rate. The zero-shot success rate is calculated by evaluating the policy acquired in CSI-27/3/9 in larger-scale new environments (such as CSI-216/24/9). We then continue to train the transferred policy in the new environment and observe the success rate after training once again in the new environment. The maximum evaluation success rate during this second training process is considered the final success rate. Fig.\ref{fig:Transferability} illustrates the transfer process.

HCGL has shown excellent performance in transferability. Firstly, HCGL has a high zero-shot success rate; the success rate only drops from 97% to 75%. We further expand the team's size to eight times (216 agents), and the zero-shot success rate is still higher than 60%. Secondly, transferred HCGL (HCGL-TF) can be trained to increase the success rate again. In all transferred tasks, HCGL-TF's final success rate was restored to above 80%.

Furthermore, as depicted in Figure 1, the number of episodes required to recover the success rate in large-scale tasks was significantly lower than training from scratch in the 27-agents task.

\textbf{Discussion.} The transferability simulations suggest that difficult large-scale tasks can be solved by addressing less difficult tasks first, then gradually increasing the number of agents and task difficulty until eventual challenges are solved. The extensible feature of ECG allows us to utilize our HCGL model in various curriculum learning methods.

\subsection{Ablation Studies.}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{img/exp_abl_gnum.pdf}
    \caption{
        An ablation study on the influence of the number of clusters.
    }
    \label{fig:ablation-num-clusters}
\end{figure}

This experiment uses CSI-21/3/9 to investigate the influence of hyper-parameter settings in the HCGL.

\subsubsection{The ablation study of clusters.}
First, we set $n_k=14$ clusters as the baseline. To investigate the influence of $n_k$, we try multiple selections of $n_k$ in task CSI-21/3/9, from $n_k=8$ to $n_k=16$. As illustrated in Fig.\ref{fig:ablation-num-clusters}, the optimal number of clusters is between 12 to 14, which roughly matches the number of invaders plus the quantity of bases in CSI-21/3/9.

\subsubsection{The ablation study of primitive actions.}
Furthermore, we test the influence of primitive actions. The baseline model uses six primitive actions, which move agents to $+x,-x,+y,-y,+z,-z$ respectively. The 14-primitive model includes additional eight directions for $(+1,+1,+1),\ (+1,+1,-1),\ \dots$, etc.

The results displayed in Fig.\ref{fig:ablation_primitive} indicate that the HCGL also works without any primitive actions, but the average success rate declined significantly. Additionally, a large number of primitive actions can also affect the performance. Increasing the operator action space can result in an increase in the required number of samples for policy exploration.\textbf{Discussion}.
Based on the simulation results presented in this section, selecting the optimal number of clusters and primitive actions is crucial for achieving optimal system performance.
The selection of an appropriate number of clusters depends on both the task at hand and the number of agents involved.
Furthermore, HCGL demonstrates superior performance when both cooperative and primitive actions are employed.

Figure \ref{fig:ablation_primitive} shows an ablation study on the influence of primitive actions. As shown, the overall performance degrades when primitive actions are removed. This observation highlights the importance of the primitive actions and their contribution to the collective action policy.

Additionally, we tested the transferability of HCGL, as shown in Figure \ref{fig:Transferability}. The policy was first trained in task CSI-27/3/9, and then the trained policy was transferred to CSI-54/6/9, CSI-108/12/9, etc. The results indicate that the policies transferred well to similar tasks with different numbers of clusters and agents. This further supports the effectiveness of HCGL for a variety of multi-agent tasks.

==> tex_polish/06-conclusion.tex.polish.tex <==
\section{Conclusions}

This paper proposes a novel MARL learning framework to address multi-agent problems that require sophisticated hierarchical collaboration. Unlike classic MARL models, we introduce a dynamic graph structure called the Extensible Cooperation Graph (ECG) to guide agents' cooperative actions. The ECG comprises three types of nodes: agents, clusters, and targets. Through dynamic edge adjustments, the ECG groups agents into clusters for carrying out either primitive individual actions or cooperative group actions. To enable such adjustments on the ECG, we assign the authority to change edge connections to four virtual operators, who have a specialized action space for manipulating the ECG and neural policy networks to acquire ECG manipulation skills through reinforcement learning.

In our experiments, we demonstrate that the ECG model not only performs well but also exhibits interpretability and transferability. Furthermore, its unique characteristic enables it to seamlessly incorporate cooperative knowledge from humans.
